Multi-megabase scale genome interpretation with genetic language models

Understanding how molecular changes caused by genetic variation drive disease risk is crucial for deciphering disease mechanisms. However, interpreting genome sequences is challenging because of the vast size of the human genome, and because its consequences manifest across a wide range of cells, tissues and scales -- spanning from molecular to whole organism level. Here, we present Phenformer, a multi-scale genetic language model that learns to generate mechanistic hypotheses as to how differences in genome sequence lead to disease-relevant changes in expression across cell types and tissues directly from DNA sequences of up to 88 million base pairs. Using whole genome sequencing data from more than 150 000 individuals, we show that Phenformer generates mechanistic hypotheses about disease-relevant cell and tissue types that match literature better than existing state-of-the-art methods, while using only sequence data. Furthermore, disease risk predictors enriched by Phenformer show improved prediction performance and generalisation to diverse populations. Accurate multi-megabase scale interpretation of whole genomes without additional experimental data enables both a deeper understanding of molecular mechanisms involved in disease and improved disease risk prediction at the level of individuals.

==> test-noneur-performance-plot.tex <==
  
  \begin{figure*}[pt!] 
  \centering
  
\figtitle{Risk Prediction for Individuals of Non-European Ancestry}
 
 \begin{subfigure}[b]{\rowheadersize\textwidth}
    \hspace{0.5em}
  \end{subfigure}
\begin{subfigure}[t]{\resultsubplotsize\textwidth}\centering
    \textsf{AUROC}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}\centering
   \textsf {AUPRC}
  \end{subfigure} 
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}\centering
    \textsf{PPV}
  \end{subfigure}\hfill 
  
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{1.5em}\textsf{Psoriasis}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_psoriasis}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_psoriasis}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_psoriasis}
  \end{subfigure}\hfill 
 
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{0.1em}\textsf{Type 1 Diabetes}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_diabetes_t1}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_diabetes_t1}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_diabetes_t1}
  \end{subfigure}\hfill  
  
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{0.1em}\textsf{Type 2 Diabetes}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_diabetes_t2}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_diabetes_t2}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_diabetes_t2}
  \end{subfigure}\hfill  
  
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{0em}\textsf{Diabetic Retino.}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_diab_eye}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_diab_eye}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_diab_eye}
  \end{subfigure}\hfill
  
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{2em}\textsf{COPD}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_copd}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_copd}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_copd}
  \end{subfigure}\hfill
 
  \begin{subfigure}[b]{\rowheadersize\textwidth}
    \rotatebox{90}{\hspace{0.5em}\textsf{Hypothyroidism}}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
  \centering
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/roc_curve_atlas_hypothyroid}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/performance/test_non_eur/pr_curve_atlas_hypothyroid}
  \end{subfigure}
  \begin{subfigure}[t]{\resultsubplotsize\textwidth}
\centering	
	\includegraphics[width=1.0\textwidth, valign=b]{figs/partialhits/test_non_eur/hit_barplot_top_atlas_hypothyroid}
  \end{subfigure}\hfill
  
\vspace{1pt}
\caption{\textbf{\themethod{} maintains better performance in predicting individual disease risk in individuals of diverse, non-European backgrounds than PRS methods.} The performance of \themethod{} compared to PRS methods in terms of Area under the Receiver Operator Curve (AUROC; leftmost column), Area under the Precision Recall Curve (AUPRC; center column) and positive predictive value among the top 3\% highest predictions (top 3\% PPV; rightmost column) on a subset of individuals of diverse, non-European ancestry. We find that \themethod{} is more transportable than PRS methods with relatively greater performance in diverse ancestries and significantly better performance also in Hypothyroidism. Stars (****) indicate statistical significance (p $\leq 0.001$, Mann-Whitney Wilcoxon test for superiority, \numprint{2000} bootstrap samples).}
\label{fig:performance_noneur}
\end{figure*}

